Learning to Guide a Saturation-Based Theorem Prover

Traditional automated theorem provers have relied on manually tuned heuristics to guide how they perform proof search. Recently, however, there has been a surge of interest in the design of learning mechanisms that can be integrated into theorem provers to improve their performance automatically. In this work, we introduce TRAIL, a deep learning-based approach to theorem proving that characterizes core elements of saturation-based theorem proving within a neural framework. TRAIL leverages (a) an effective graph neural network for representing logical formulas, (b) a novel neural representation of the state of a saturation-based theorem prover in terms of processed clauses and available actions, and (c) a novel representation of the inference selection process as an attention-based action policy. We show through a systematic analysis that these components allow TRAIL to significantly outperform previous reinforcement learning-based theorem provers on two standard benchmark datasets (up to 36% more theorems proved). In addition, to the best of our knowledge, TRAIL is the first reinforcement learning-based approach to exceed the performance of a state-of-the-art traditional theorem prover on a standard theorem proving benchmark (solving up to 17% more problems).

==> app-hyperparam.tex <==
\section{Appendix - Hyper-Parameter Tuning}
We used gradient-boosted-tree  search  from
scikit-optimize~\footnote{https://scikit-optimize.github.io/} to  find  effective  hyper-parameters using 10\% of of Mizar40 dataset. We present here the list of hyper-parameters as well as their value range provided as input to the hyper-parameter tuning algorithm. We also  present the list of all hyper-parameter values used in our experiments.

\begin{table*}
  \caption{Hyper-Parameter Ranges and Values Used } 
  \label{tab:hyperparams_tunable}
  \centering
  \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{|l|l|l|}
        \hline
        Name & Value Range & Value Used\\  \hline
        $k$ (number of layers) & Integer([0, 30]) & 2 \\
        Units per layer & Integer([25, 200]) & 161 \\
        Activation function & \{ReLU\} & ReLU \\ 
        $2d$ (sparse vector size) &  Integer([10, 1000]) &  645 \\
        Dropout probability & Real([0, 0.6]) &  0.57 \\
        $\lambda$ (entropy reg.) & \{0.0, 0.002, 0.004, 0.008, 0.016, 0.032, 0.064, 0.128\} & 0.004 \\
        $\tau$ (temperature) & Real([1, 5])  & 1.13\\
        $\tau_0$ (temperature threshold) & Integer([10, 50]) & 11 \\
        Temperature decay factor & Real([.95, 1]) & 0.9998\\
        $\rho$ (expert reliance decay) & Real([0.1, 0.99]) & 0.75 \\
        Reward Normalization & \{No Norm, Norm. w.r.t. Beagle #steps, Relative Norm. w.r.t. best attempt\} & No Norm \\
        Treat constants as functions in vectorization & \{TRUE, FALSE\} & TRUE\\ 
        Optimizer & \{Adam(betas = (0.9, 0.999), weight decay = 0, eps = 10^{-8})\} & Adam \\
        Learning rate & \{0.001\} & 0.001  \\
        Batch size & \{32\} & 32 \\
        Number of epochs & \{15\} & 15 \\
        $w$ (keep examples from the last $w$ iterations) & \{20\} & 20 \\
        \hline
    \end{tabular}
    }
\end{table*}

Table~\ref{tab:hyperparams_tunable} below shows the list of   hyper-parameters. For each hyper-parameter, we show  its value range and the value used in our experiments. 




==> sections/4experiments.tex <==
\section{Experiments and Results}
\label{sec:experiments}







\subsection{Datasets}
We used two standard, benchmark datasets to evaluate \trail's effectiveness: \emph{M2k}~\cite{KalUMO-NeurIPS18-atp-rl} and \emph{MPTP2078}~\cite{alama2014premise} (referenced as MPTP going forward). Both M2k and MPTP are exports of parts of Mizar\footnote{\url{https://github.com/JUrban/deepmath/}}~\cite{mizar} into the TPTP~\cite{tptp} format. The M2k dataset contains 2003 problems selected randomly from the subset of Mizar that is known to be provable by existing ATPs, whereas MPTP is a set of 2078 Mizar problems selected regardless of whether or not they could be solved by an ATP system. 
% \emph{TPTP}\footnote{\url{http://tptp.cs.miami.edu/}} is the definitive benchmarking library for theorem provers, designed to test ATP performance across a wide range of problem domains (e.g., biology, geography, number theory, etc.). 
% The different problem domains within the TPTP will serve as our data-sparse setting in our transfer experiment, as each distinct problem domain within the TPTP has on average only 400 problems. 
% %\footnote{\url{http://www.tptp.org/Seminars/TPTP/Synopsis.html}}
% % Problems from Mizar were drawn from the subset used by \cite{Alemi-NIPS16-deepmath}, i.e. the subset of problems known to be solvable by existing ATPs (this subset was used to allow for a direct comparison against our baselines). 
% For comparison against other ATP systems, we used the \emph{M2k}~\cite{KalUMO-NeurIPS18-atp-rl} and \emph{MPTP2078}~\cite{alama2014premise} datasets. The M2k dataset contains 2,003 problems selected randomly from the subset of Mizar that was known to be provable by existing ATPs. MPTP2078 is another set of Mizar problems, however problems in this set were selected regardless of whether or not they could be solved by an ATP system. 

% For our generalization experiment, we added a random subset of 2,000 problems from the TPTP dataset selected from various problem domains (coined \emph{TPTP}). TPTP\footnote{\url{http://tptp.cs.miami.edu/}} is the definitive benchmarking library for theorem provers, designed to test ATP performance across a wide range of problem domains. This was done to measure how well the proof strategies learned by \trail on Mizar could generalize to problems less likely to require purely equational reasoning, as TPTP includes a broad range of distinct problem domains (e.g., common sense reasoning, software verification, etc.).

\subsection{Implementation Details}
The current implementation of \trail assumes only that its underlying reasoner is saturation-based and is otherwise reasoner-agnostic. It defines an API that can be implemented by any reasoner to allow \trail to act as its proof guidance system. {\color{red}Shajith: can we add more here about the interface itself?} Throughout all experiments presented in the following sections, the reasoner in use has its own proof guidance completely disabled when integrated with \trail. Whenever the reasoner reaches a decision point, it delegates the decision to \trail's policy to choose the next action to pick. Using an off-the-shelf reasoner (like Beagle~\cite{Beagle2015} or E-prover~\cite{eprover}) to execute inferences ensures that the set of inference rules available to \trail are both sound and complete, and that all proofs generated can be trusted. To empirically validate our claims of reasoner-agnosticism, we have integrated \trail with two different saturation-based theorem provers, Beagle~\cite{Beagle2015} and E-prover~\cite{eprover}. %In future work, we intend to integrate with other reasoners for sequent calculus and higher order logic. 

\subsection{Hyperparameters}


\begin{table}[]
\centering
\begin{tabular}{lccc}
\toprule
                    & \trail (Beagle backend) & \trailplus (E backend) &  \\
\midrule
Chain               & 653                    &      956             &  \\
Term Walks              & 737                    &      967               &  \\
Chains + Term Walks  & \bf 910                    & \bf 1024              & \\
\bottomrule
\end{tabular}
\caption{Performance of {\trail} (using two different backends)  with multiple sparse vectorizers on MPTP benchmark}
\label{sparse_E_exp}
\end{table}

\subsection{Choice of Sparse Vectorizer and Underlying Reasoners}
The term walk and chain-based vectorization modules used by \trail  are intended to quickly extract structural features from their inputs. Though they are not tailored to any particular domain within FOL, they are clearly feature engineering. 
We view \trail as providing a framework for further testing this (we show a detailed analysis in Section~\ref{gnn_exps} for a comparison against multiple GNN vectorizers).

We start our experiments from the best reported setting in the previous TRAIL version \cite{crouse2019deep}. In particular, Table~\cite{sparse_E_exp} shows the performance of TRAIL using Chain + Engima; the best performing vectorizer according to \cite{crouse2019deep} when using Beagle as its back-end reasoner on MPTP datasets. We also show the performance of best Chain + Enigma vectorizer in TRAIL++ as we use E as the underlying reasoner. As the results show, using E resulted in solving more problems and TRAIL++ was able to collect a larger set of examples that resulted in a better policy network. Doing this resulted in solving 114 problems (~5\%) improvement. We also noticed a similar improvement in M2K dataset.
This experiment validate our claim that this approach is indeed reasoner agnostic and can be generally used to guide existing theorem provers. In the rest of this section, all TRAIL++ experiments are using E-prover as its underlying reasoner. 

\begin{table}[]
\centering
\begin{tabular}{ll}
\toprule
                                            & MPTP-2078b  \\
\midrule
TRAIL++                                       & 1024  \\
TRAIL++  w/ Bounded Rewards                    &   1051       \\
TRAIL++  w/ Bounded Rewards + Exploration & \bf 1095   \\
\bottomrule
\end{tabular}
\caption{Performance (best iteration) with minimum/maximum rewards and more exploration using Chains + Term Walks vectorizer}
\label{reward_exploration}
\end{table}


\subsection{Bounded Rewards and Exploration Effect}
In this experiment, we use the best setting from above experiment; i.e. using E-prover as the underlying reasoner and Term Walks + Chains as the vectorizer. We then test the effect of using bounded rewards and more exploration. In particular, we set the minimum reward to be 1.0 where the maximum reward to be 2.0. A reward value of 2.0 means TRAIL++ was able to solve the problem twice as fast compared to E-prover. {\color{red} Elaborate as in what this means for encouraging TRAIL to solve more and more problems even if they are not very fast}. As Table~\ref{reward_exploration} shows, bounded rewards clearly helped TRAIL++ to solve more problems on the hard dataset MPTP-2078b (27 more problems). As we allow TRAIL++ to explore the search space more over iterations (54), {\color{red} TRAIL++ was able to solve even more problems (54). This clearly shows ... Add parameters values and their meaning.}. 






\label{gnn_exps}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}lcc|cc@{}}
\toprule
                                                & \multicolumn{2}{c|}{MPTP}                                             & \multicolumn{2}{c}{M2k}                                              \\ \cmidrule(l){2-5} 
                                                & \multicolumn{1}{l}{Best Iteration} & \multicolumn{1}{l|}{Commulative} & \multicolumn{1}{l}{Best Iteration} & \multicolumn{1}{l}{Commulative} \\ \midrule
\multicolumn{1}{l|}{Chains + Term Walks}            & 1095                               & 1155 (\small 185)                       & 1732                               & 1765 (\small 46)                       \\
\multicolumn{1}{l|}{PreTrainedGCN}              & 1020                               & 1092 (\small 139)                       & 1686                               & 1733 (\small 34)                       \\
\multicolumn{1}{l|}{GCN (vanilla)}              & 892                                & 998 (\small 101)                        & 1610                               & 1684 (\small 23)                       \\
\multicolumn{1}{l|}{GCN (topological batching)} & \textbf{1159}                               & \textbf{1199 (\small 218)}              & \textbf{1776}                               & \textbf{1800 (\small 49)}              \\
% \multicolumn{1}{l|}{GCN (topological batching)} & \textbf{1167}                               & \textbf{1213 (\small 228)}              & \textbf{1776}                               & \textbf{1808 (\small 50)}              \\
\multicolumn{1}{l|}{SAGE}                       & 1061                               & 1150 (\small 186)                       & 1678                               & 1739 (\small 36)                       \\ \bottomrule
\end{tabular}
\caption{Number of problems solved by different vectorizers. The number in brackets denotes the number of problems solved by TRAIL and not by E.}
\label{sparse_vs_neural}
\end{table*}






\subsection{Graph Neural Networks Based Vectorization}


In this section, we compare the performance of various graph neural network vectorizations techniques compared to the best performing sparse vectorizer (Chain + Term Walks). In particular, we show the individual performance of {\trail} using each vectorizer, detailed analysis of the results and test transfer learning across datasets. 

\subsubsection{Sparse vs. Neural Vectorizers}
Table~\ref{sparse_vs_neural} shows the performance of TRAIL using its best sparse vectorizer (Chains + Term Walks) against 4 graph based vectorizers (see Section ~\ref{}) on the the two dataset benchmarks. For each vectorizer, we report both the best number of problems solved at any iteration and the union of all problems solved across iterations (cumulative). The numbers in brackets indicated the number of problems solved by TRAIL++ with this vectorizer which E-prover itself could not solve with 100 seconds. Off the shelf GCN vectorizers solved the least number of problems across both datasets. More advanced models such as SAGEGCN did much better in terms number of the overall problems solved (1102 on MPTP and 1696 on M2k) and how many problems it solved better than E itself (157 on MPTP and 27 on M2K). Surprisingly, the Pre-Trained vectorizer performed very well although it has not been finetuned at all for theorem proving and it does not even capture the full vocabulary {\color{red} Explain}. As Table\ref{sparse_vs_neural} also shows, our own GCN vectorizer which takes into account the DAG nature of logical formulas and features a skip connections and layer normalization performs the best among all these verctorizers. {\color{red} A statistical significance test shows .. over Chain + Term Walks} 




\begin{figure*}[ht]
\begin{subfigure}
  \centering
  % include first image
  \includegraphics[width=.45\linewidth]{figures/2078b_completition_ratio.pdf}  
%   \caption{Put your sub-caption here}
  \label{fig:sub-first}
\end{subfigure}\hfill
\begin{subfigure}
  \centering
  % include second image
  \includegraphics[width=.45\linewidth]{figures/2078b_time_improv.pdf}  
%   \caption{Put your sub-caption here}
  \label{fig:sub-second}
\end{subfigure}
\caption{MPTP2078b: Completion Ratio and Time Improvement of different vectorizers}
\label{fig:2078b_compl_time}
\end{figure*}

\begin{figure*}[ht]
\begin{subfigure}
  \centering
  % include first image
  \includegraphics[width=.45\linewidth]{figures/m2k_completition_ratio.pdf}  
%   \caption{Put your sub-caption here}
  \label{fig:sub-first}
\end{subfigure}\hfill
\begin{subfigure}
  \centering
  % include second image
  \includegraphics[width=.45\linewidth]{figures/m2k_time_improv.pdf}  
%   \caption{Put your sub-caption here}
  \label{fig:sub-second}
\end{subfigure}
\caption{M2K: Completion Ratio and Time Improvement of different vectorizers}
\label{fig:m2k_compl_time}
\end{figure*}




\subsubsection{Time Improvement and Completion Ratio}
Figures \ref{fig:2078b_compl_time} and \ref{fig:m2k_compl_time} show the completion ratio and time improvement for all vectorizers across iterations. The completion ratio captures the percentage of problems solved in each dataset per iteration. Time improvement shows how fast TRAIL++ solved a problem compared E-prover on average. 

{\color{red} Discuss stability and best performing vectorizer, imporvement across iterations .. . Mention also that 8 times faster than E is a BIG DEAL}


% \begin{figure*}[ht]
% \begin{subfigure}
%   \centering
%   % include first image
%   \includegraphics[width=.45\linewidth]{figures/2078b_nnet_training.pdf}  
% %   \caption{Put your sub-caption here}
%   \label{fig:sub-first}
% \end{subfigure}\hfill
% \begin{subfigure}
%   \centering
%   % include second image
%   \includegraphics[width=.45\linewidth]{figures/M2k_nnet_training.pdf}  
% %   \caption{Put your sub-caption here}
%   \label{fig:sub-second}
% \end{subfigure}
% \caption{Policy Training Times for different vectorizers: MPTP-2078b (left) and M2K (right)}
% \label{fig:nnet_training}
% \end{figure*}

\subsubsection{Graph Vectorization Time}


% \subsubsection{Neural Network Training Time}
% In this experiment, we show the overall neural network training time. This network includes both the vecorizer network as well as the policy network. In all vectorizers, the training time increases across iterations and TRAIL++ keeps accomulating more examples at the end of iteration and keeps them in its history of examples collected. As Figure~\ref{fig:nnet_training} shows, updating the vectorizer network seem to dominate the overall training time.  This is clear when the vectorizer network is only few feed forward layers (Chain + Term Walks) or the vectorizer model does not get updated at all (PreTrained). On the other hand, GCN (vanilla) and SAGE seem to require a lot of time to converge where the training time keeps increasing significantly across iterations. GCN with topological batching seems to acheive the right mix of performance and runtime efficiency. {\color{red} Elaborate}   


\subsubsection{Transfer Across Datasets}
Table~\ref{{tab:transfer}} also shows the performance of TRAIL++ when trained on M2k and tested on MPTP dataset, and vice versa for all 5 vectorizers {\color{red} best or cummulative?}. In terms of transfer, Chain + Term Walks, PreTrained and GCN with topological batching vectorizers all showed good transfer across both datasets with GCN with topological producing the best results. This provides evidence that these features are reasonably domain-general (though, we again emphasize that, while M2k and MPTP are different datasets and may require different reasoning strategies, they are both generated from Mizar). {\color{red}Notably, there was only a 11\% loss of performance when training on MPTP and testing M2K, and a 3\% loss when training on M2k and testing MPTP2078. From this experiment we conclude that cheap structural features, though hand-engineered, are relatively domain-general, which again will make them tough for more complex approaches to beat.}

\begin{table}
\centering
\begin{tabular}{lcc}
\toprule
     & \multicolumn{1}{l}{MPTP $\rightarrow$ M2K} & \multicolumn{1}{l}{M2K $\rightarrow$ MPTP}    \\
\midrule
Chains + Term Walks   & 1623      & 969    \\
PreTrainedGCN  & 1643     & 927\\
GCN (vanilla) & 1602 & 732 \\
GCN (topological batching) & \bf 1674     & \bf 1048 \\
SAGE  & 1649    & 871 \\
\bottomrule
\end{tabular}
\caption{Transfer Across Datastes: Performance (number of problems) of models trained on MPTP and tested on TPTP and vice versa.}
\label{tab:transfer}
\end{table}

% In this experiment, we measure the performance of {\trail} on MPTP2078 across different sparse vectorization techniques and different underlying reasoners. In particular, we tested Chain patterns, Enigma walks and their combination when using {\trail} to guide Beagle and E reasoners. 


% To choose the best sparse vectorizer, we performed an experiment where we varied the vectorization modules available to \trail, comparing three different ablated versions: 1) \trail using the chain-based vectorizer, 2) \trail using the term walk vectorizer \cite{JU-CICM17-enigma}, and 3) combinations of these vectorizers. For all ablations, \trail had access to the general-purpose vocabulary-independent features %(e.g., age, literal count, etc.)
% mentioned in Section \ref{sec:vectorization}.

% We report \trail's performance using both the prior \emph{best iteration performance} metric (where the train and test sets are the same).  Table~\ref{sparse_exp} shows the performance of \trail on MPTP benchmark. Examining Table \ref{vect_transfer}, we see that while chain-based vectorization is weaker than term walk vectorization, the combination of the two achieves significantly better results as a whole. This suggests that they are capturing non-redundant feature sets. Furthermore, {\trail} with E as its underlying reasoner is much stronger in terms of number of problems solved across all vectorizers; an expected behaviour given the superior of standalone E prover compared to Beagle. 

% \subsection{Choice of Reward Structure}
% We explored two variations of reward structures in {\trail}. The first one is based on the number of steps found to find the proof. While this reward captures well the intrinsic difficulty of the problem, it does not model the complexity of individual steps. Certain proof steps may require more time to execute by the reasoner and may also inflate the search space more than others. Therefore, we also explored another reward based on the overall time needed to obtain the proof. Our hypothesis is that the time based reward is more inclusive of all other factors that may affect the underlying reasoner such as step complexity and the size of the search space. Finally, as mentioned in Section \ref{sec:rl_formulation}, we also normalize the reward obtained by using problem difficulty obtained from traditional reasoners; E in this experiment. Table \ref{reward_structure} shows TRAIL's performance on MPTP benchmark with both reward types without and without normalization. As the results show, normalization and time-based reward are more efficient in guiding TRAIL towards solving more problems.  





%ibrahim@trail91:/disk0/Trail$ grep "^10" /disk0/Trail/2078b_E_time_herbrand2500_Mar17/selfplay_train_details.tsv | grep -v "1e-08" | wc -l
% 956
% ibrahim@trail100:~$ grep "^10" /disk0/Trail/2078b_E_time_enigma2500_Mar17/selfplay_train_details.tsv | grep -v "1e-08" | wc -l
% 967



% \begin{table}
% \centering
% \begin{tabular}{lrr}
% \toprule
%           & \multicolumn{1}{l}{w/o Normalization} & \multicolumn{1}{l}{w/ Normalization}  \\
% \midrule
% Step based &             963                          &                  997                     \\
% Time based &              1,015                         &              \bf 1,030                         \\
% \bottomrule
% \end{tabular}
% \caption{Choice of reward structure on MPTP dataset using Chains + Enigma vectorizer}
% \label{reward_structure}
% \end{table}


\subsubsection{GCN with topological batching: Ablation Study}

In this experiment, we vary the embedding size for the best performing vectorizer; GCN topological batching. In prticular, we vary clause and action embedding sizes between 64, 128, 256 and 512. Table~\ref{tab:embed_size} shows the performance on both datasets.  Lower embedding dimensions are preferred in our setting since it means less number of weights to learn and accordingly faster training and inference times. Table~\ref{tab:embed_size} clearly shows this aspect where embedding sizes 64 and 128 clearly outperform 256 and 512 on MPTP-2078 with 64 being the best overall across both datasets. Accordingly, we use this best performing setting in the rest of our experiments. 

% gcn_top_64:
% best_iter:  ('18', 1167)
% last_iter ('20', 1162)
% Total number of probled solved (commulative):  1213
% Total number of probled solved by TRAIL and not by E within 100s:  228
% best_iter:  ('15', 1776)
% Total number of probled solved (commulative):  1808
% Total number of probled solved by TRAIL and not by E within 100s:  50

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\begin{tabular}{lll}
\toprule
 Embedding Size   & 2078b & M2k  \\
% \midrule
% E           &  1,036        & 1,819    \\
% Beagle      & 742        & 1543      \\
\midrule
512 & 1199  & 1800 \\
256 & 1189  & 1807 \\
128 & \bf 1215  & 1800 \\
64  & 1213  & \bf 1808\\
\bottomrule
\end{tabular}%
\caption{GCN with topolgical batching performance (number of problems solved (cumulative)) various clause embedding sizes}
\label{tab:embed_size}
\end{table}

In the next experiment, we test the effect of a number of design decision we picked for GCN with toplogical batching, namely effectivness of skip connections, layer normalization and read-out function for formula embeddings, whether it is based on reading the formula root only or averaging over the whole graph nodes. Using an embedding size of 64, Table~\ref{tab:ablation}  shows the performance as we switch off these options on MPTP-2078 dataset.  

\begin{table}[]
\centering
\begin{tabular}{lll}
\toprule
   & 2078b & M2k  \\
% \midrule
% E           &  1,036        & 1,819    \\
% Beagle      & 742        & 1543      \\
\midrule
Full & 1213  & 1808 \\
No Skip Connections &   &  \\
No Root Readout &    &  \\
No Layer Normalization &    &  \\

\bottomrule
\end{tabular}%
\caption{Ablation study of GCN with topolgical batching in terms of  (number of problems solved (cumulative)}
\label{tab:ablation}
\end{table}


{\color{red}MAKE Table~\ref{tab:m2k_2078} all with commulative numbers? or both}
\begin{table}[t]
 \centering
\footnotesize
\begin{tabular}{l l c c}
\toprule
 & & M2k & MPTP2078  \\
\toprule
% \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Traditional}}&Beagle~\cite{Beagle2015} & 1,543 & 742 \\
% & E~\cite{schulz2002brainiac} & 1,922 &  998\\
\multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Traditional}}& E & \bf 1,819  &  \bf 1,036\\
&Beagle & 1543 & 742 \\
& mlCop & 1034 & 502\\
% E           &  1,036        & 1,819    \\
% Beagle      & 742        & 1543      \\

\midrule
\multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Reinforcement \\ Learning-Based}}& rlCop &  1235 & 733 \\
& plCop & 1359 & 782 \\
% &\trail & 1,520 & 786 \\
% &\trail (w/ conjecture) & 1,459 & 819 \\
&\trail  & 1561 & 910 \\
&TRAIL++  & \bf{1,808} & \bf{1,213} \\
\bottomrule
\end{tabular}
\caption{Number of problems solved in M2k and MPTP2078. 
Best two approaches in bold
}
\label{tab:m2k_2078}
\end{table}

% \subsection{Effectiveness of \trail}

% % For traditional ATP systems, we compare \trail to: 1) E~\cite{schulz2002brainiac} in auto mode, a state-of-the-art saturation-based ATP system that has been under development for over two decades, 2) Beagle~\cite{Beagle2015}, a newer saturation-based theorem prover that has achieved promising %(but not yet state-of-the-art)
% % results in recent ATP competitions, and 3) mlCop \cite{kaliszyk2015certified}, an OCaml reimplementation of leanCop \cite{otten2003leancop}, which is a tableau-based theorem prover that was applied to M2k in \cite{KalUMO-NeurIPS18-atp-rl} and MPTP2078 in \cite{zombori2020prolog}. For learning-based approaches, we compare against two recent RL-based approaches: rlCop ~\cite{KalUMO-NeurIPS18-atp-rl} and plCop~\cite{zombori2020prolog}, both of which are connection tableau-based theorem provers that build off mlCop and leanCop, respectively. 
% % All results for mlCop, rlCop, plCop, and E are those reported in \cite{KalUMO-NeurIPS18-atp-rl,zombori2020prolog}, except for E on M2k which we ran ourselves. We also replicated plCop and rlCop numbers under our exact hardware and time constraints and found comparable results.   
% % % We report all the hyperparameters for \trail in Appendix A.1
% % % along with an overview of the underlying reasoner (Beagle) \trail uses to execute its selected actions (Appendix A.2).
% % %We also describe in Appendix \ref{sec:underlying_reasoner} the underlying reasoner (Beagle) \trail uses to execute its selected actions.

% In this experiment, we compare against two recent RL-based approaches: rlCop (\cite{KalUMO-NeurIPS18-atp-rl}) and plCop (\cite{zombori2020prolog}), both of which are connection tableau-based theorem provers that build off mlCop and leanCop, respectively.  
% All results for rlCop, plCop are those reported in \cite{KalUMO-NeurIPS18-atp-rl,zombori2020prolog}. We also replicated plCop and rlCop numbers under our exact hardware and time constraints and found comparable results.   
% Following \cite{KalUMO-NeurIPS18-atp-rl,zombori2020prolog}, we report the \textit{best iteration completion performance}. In this setting, \trail starts from scratch and is  applied to M2k and MPTP2078 for 10 iterations, with learning from solved problems occurring after each iteration completes. The reported number of problems solved is then the number solved in the best performing iteration.



% \begin{table}[t]
%  \centering
% \footnotesize
% \begin{tabular}{l l c c}
% \toprule
%  & & M2k & MPTP2078  \\
% \toprule
% % \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Traditional}}&Beagle~\cite{Beagle2015} & 1,543 & 742 \\
% % & E~\cite{schulz2002brainiac} & 1,922 &  998\\
% \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Traditional}}& E & \bf 1922 &  \bf 998\\
% &Beagle & 1543 & 742 \\
% & mlCop & 1034 & 502\\

% \midrule
% \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Reinforcement \\ Learning-Based}}& rlCop &  1235 & 733 \\
% & plCop & 1359 & 782 \\
% % &\trail & 1,520 & 786 \\
% % &\trail (w/ conjecture) & 1,459 & 819 \\
% &\trail  & \bf{1561} & \bf{910} \\
% \bottomrule
% \end{tabular}
% \caption{Number of problems solved in M2k and MPTP2078. %TRAIL numbers are with 100 seconds time limit. 
% Best two approaches in \textbf{bold}
% }
% \label{tab:m2k_2078}
% \end{table}

% \begin{table}[t]
%  \centering
% % \footnotesize
% \begin{tabular}{l c c c}
% \toprule
% & M2k & MPTP2078 & TPTP  \\
% \midrule
% % \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Traditional}}&Beagle~\cite{Beagle2015} & 1,543 & 742 \\
% % & E~\cite{schulz2002brainiac} & 1,922 &  998\\

% rlCop &  1,235 & 733 & -- \\
% plCop & 1,359 & 782 & -- \\
% % &\trail & 1,520 & 786 \\
% % &\trail (w/ conjecture) & 1,459 & 819 \\
% \trail (Beagle backend) & \bf{1,561} & \bf{910} &  671 \\
% \trail (E backend) & \bf{1,652} & \bf{1030} &  725\\

% \bottomrule
% \end{tabular}
% \caption{Learning based approaches: Number of problems (best iteration) solved in M2k and MPTP2078 datasets. 
% Best two approaches in \textbf{bold}
% }
% \label{tab:m2k_2078}
% \end{table}

% Table~\ref{tab:m2k_2078} shows the performance of \trail against both traditional ATP systems and recent learning-based approaches. Following~\cite{zombori2020prolog}, we limit TRAIL to a maximum of 2,000 steps per problem with a hard limit of 100 seconds. As Table~\ref{tab:m2k_2078} shows, while \trail outperformed Beagle, state-of-the-art saturation-based ATP systems are still superior to RL-based systems, with E solving the most problems on both datasets. Among learning-based approaches, \trail\ solved 202 more problems on M2k compared to plCop~\cite{zombori2020prolog}, and on MPTP2078, \trail\ solved 128 more problems. On both datasets \trail outperformed its underlying reasoner, Beagle, with a 22\% relative improvement on MPTP2078. These results show that \trail (when trained from a random initial policy) is a competitive theorem proving approach, as it outperformed all other systems except for E, with significant gains over prior RL-based approaches. Notably, \trail substantially narrows the gap between state-of-the-art traditional and from-scratch RL approaches on MPTP2078.

\subsection{Effectiveness of TRAIL}
Table~\ref{tab:m2k_2078} shows the performance of \trail against both learning-based approaches. Following~\cite{zombori2020prolog}, we limit TRAIL to a maximum of 2,000 steps per problem with a hard limit of 100 seconds. As Table~\ref{tab:m2k_2078} shows, when using Beagle as its underlying reasoner (with no decision making), \trail\ solved 202 more problems on M2k compared to plCop~\cite{zombori2020prolog}, and on MPTP2078, \trail\ solved 128 more problems. When using E, which is known to be more efficient by itself than Beagle, \trail\ outperforms both rlCop and plCop by an even bigger margin; 293 on M2k and 248 on MPTP. 
% On both datasets \trail outperformed its underlying reasoner, Beagle, with a 22\% relative improvement on MPTP2078. 
These results show that \trail (when trained from a random initial policy) is a competitive theorem proving approach with significant gains over prior RL-based approaches. {\color{red} We show comparison aganist traditional theorem provers E and Beagle in Section~\ref{}} 


% set iterations to 20
%------------on both M2078b and M2k datasets-----





% \subsection{Value of Attention Over Processed Clauses}

% % {\color{blue}
% As refuting the conjecture is the end goal of proof search, incorporating the negated conjecture into action selection has clear value.
% % } 
% However, we would expect processed clauses to be useful as well, since most inferences will involve premises from both the unprocessed and processed clauses. To determine the utility of including processed clauses in action selection, we performed an ablation experiment that restricted \trail to utilizing \emph{only} the conjecture's neural representation in the processed clause matrix (i.e., the embedded representation for each processed clause became $\hat{\mathbf{h}}^{(p)}_i = \mathbf{h}^{(c)}$). This turned the attention mechanism into a measure of how aligned an action was to solely the conjecture representation.

% When using only the conjecture representations, \trail solved 1,561 problems on M2k and 854 problems on MPTP. Recall that \trail when incorporating processed clause and conjecture representations solved 1,561 problems on M2k and 910 problems on MPTP. Though there was no difference for M2k, it is significant that \trail could solve 56 more problems ($\sim$6\% relative improvement) on MPTP when incorporating processed clauses.  {\color{red}Repeat experiment on E}
%It shows that, in certain cases, performance is being left on the table 



%-------------------------------------------------------%

% \begin{table*}
% \centering
% \begin{tabular}{llll}
% \toprule
%  & \multicolumn{1}{l}{MPTP} & \multicolumn{1}{l}{M2k} & \multicolumn{1}{l}{TPTP}  \\
% \midrule
% E           & \bf 1,036        & \bf1,819      & \bf1,504     \\
% Beagle      & 742        & 1543      & 839      \\
% \midrule
% HE          & \bf 1,070 \small{(133)} & \bf1,717 \small{(33)} & \bf 958 \small{(1)}  \\
% PreTrainedGCN          & 983 \small{(83)} & &  \\
% % PreTrainedGCN          & 983 \small{(83)} & 1,553 \small{(16)} & 745 \small{(0)}  \\
% GCN         & 959 \small{(93)}   & 1,605 \small{(19)} & 887 \small{(0)}  \\
% SGCN        & 874 \small{(70)}   & 1,258 \small{(1)}  & 863 \small{(0)}  \\
% SAGE        & 941 \small{(97)}   & 1,656 \small{(24)} & 774 \small{(0)}  \\
% GAT         & 742 \small{(22)}   & 1,303 \small{(4)}  & 620 \small{(0)} \\
% \bottomrule
% \end{tabular}
% \caption{Cumulative number of problems solved by different vectorizers. The number in brackets denotes the number of problems solved by TRAIL and not by E.}
% \label{sparse_vs_neural}
% \end{table*}

% \subsection{Sparse vs. Neural Vectorizers}
% In this section, we compare the performance of various graph neural network vectorizations techniques compared to the best performing sparse vectorizer (Chain + Term Walks). In particular, we show the individual performance of {\trail} using each vectorizer, detailed analysis of the results, transfer across datasets and problem domains. 

% Table~\ref{sparse_vs_neural} shows the performance of TRAIL using its best sparse vectorizer (HE) against 5 graph based vectorizers (see Section ~\ref{}) on the three benchmarks. We also compare to traditional theorem provers E and Beagle. Compared to state-of-the-art E-prover, \trail\ with HE vectorizer solved 34 more problems in total. Among all problems solved by \trail\, 133 are problems that E never solved within the 100 seconds time limit (~12\%). \trail\'s performance on M2K is slightly inferior compared to E, but better than Beagle. On TPTP, \trail is again better than Beagle but much worse than E's performance. {\color{red}This is due to .. }. 

%-------------------------------------------------------%








% \subsection{Generalization to Data-Sparse Problem Domains}



% \begin{table}[]
% \centering
% \begin{tabular}{llllll}
% \toprule
%     & Chains + Enigma  & GCN & SAGE & SGCN & GAT \\
% \midrule
% SET & \bf 161 & 144 & 80   & 128  & 105 \\
% GEO & \bf 101 & 75  & 86   & 85   & 65  \\
% SWC & 42  & \bf 54  & 35   & 38   & 14  \\
% SWV & \bf 85  & 58  & 29   & 55   & 52  \\
% CSR & 66  & 50  & 58   & \bf 73   & 56  \\
% KLE & 15  & \bf 23  & 18   & 16   & 9   \\
% LCL & 11  & \bf 23  & 7    & 21   & 16  \\
% SEU & \bf 52  & 38  & 27   & 29   & 30  \\
% SWB & 29  & 26  & \bf 32   & 29   & 29  \\
% KRS & \bf 32  & 29  & 30   & 30   & 29  \\
% SYN & 25  & 25  & 25   & 25   & 24  \\
% GRP & 8   & \bf 16  & 10   & 9    & 10 \\
% \bottomrule
% \end{tabular}
% \caption{Number of problems solved across top-10 problem domains in TPTP dataset when solved using an MPTP trained model (\textit{transfer experiment})}
% \label{tab:tptp_exps}

% \end{table}



% Table \ref{tab:tptp_exps} shows \trail's performance when it is trained on MPTP  and tested on distinct problem domains
% %\footnote{\url{http://www.tptp.org/Seminars/TPTP/Domains.html}}
% within TPTP. The subject matter between domains within TPTP can vary greatly. For instance, CSR tests common sense reasoning, while GEO involves reasoning about geometry, and SWC covers software verification. This results in different needs between domains, e.g., the CSR domain requires heavy use of the resolution inference rule while the GEO domain involves more equational reasoning and thus requires the superposition inference rules. {\color{red}By training on Mizar (a completely different dataset with different symbols designed for different purposes), \trail was able to nearly match Beagle in many categories. Furthermore, the performance of the untrained, random model shows that \trail was clearly learning transferable proof search strategies.}




% \begin{figure*}
% \begin{center}
% % \centerline{\includegraphics[width=\columnwidth]{figures/fig1.pdf}}
% \includegraphics[width=0.7\textwidth]{figures/successful_2078b_vectorization.pdf}
% \caption{Vectorization times normalized by number of steps for successful proof attempts (MPTP-2078b)}
% % \vspace{-0.1in}
% \label{fig:vec_times}
% \end{center}
% \end{figure*}


% \begin{figure*}
% \begin{center}
% % \centerline{\includegraphics[width=\columnwidth]{figures/fig1.pdf}}
% \includegraphics[width=0.7\textwidth]{figures/successful_2078b_reasoning_times.pdf}
% \caption{Time spent on reasoning by different vectorizers  (MPTP-2078b)}
% % \vspace{-0.1in}
% \label{fig:reason_times}
% \end{center}
% \end{figure*}





% \begin{figure*}[ht]
% \begin{subfigure}
%   \centering
%   % include first image
%   \includegraphics[width=.45\linewidth]{figures/2078bsuccessful_step_taken_.pdf}  
% %   \caption{Put your sub-caption here}
%   \label{fig:sub-first}
% \end{subfigure}\hfill
% \begin{subfigure}
%   \centering
%   % include second image
%   \includegraphics[width=.45\linewidth]{figures/2078bfailed_step_taken_.pdf}  
% %   \caption{Put your sub-caption here}
%   \label{fig:sub-second}
% \end{subfigure}
% \caption{Distribution of number of steps taken by TRAIL with different vectorizers on MPTP-2078b}
% \label{fig:fig}
% \end{figure*}













% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t]
% \centering
% \footnotesize
% \begin{tabular}{llcc cc}
% \toprule
%                                   &                      & \multicolumn{2}{c}{No Transfer} & \multicolumn{2}{c}{Transfer}                  \\
% \cmidrule(l{2pt}r{2pt}){3-4}\cmidrule(l{2pt}r{2pt}){5-6}
%                                   &                      & M2k               & MPTP   & MPTP $\rightarrow$ M2k & M2k $\rightarrow$ MPTP  \\
% % \cmidrule{3-6}
% \midrule
% % \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}~~~~~Sparse \\ Vectorization\end{tabular}}           & Chains               &   1473	     &   653       &    1463      &    418  \\
% \multirow{3}{*}{Sparse Only}           & Chains               &   1473	     &   653       &    1463      &    418  \\

%                                   & Term Walks                &  1552	     &   737        &   1425      &     570 \\
%                                   & Chains + Term Walks       &  \bf 1561         &  \bf 910  &  \bf 1510     &   \bf 812\\
% \midrule
% Neural  Only                   & GCN                  &  1523	     &   750       &   1394     &     712 \\
% \midrule
% \multirow{3}{*}{Sparse \& Neural} &  GCN + Chains         &    1495          &    734      &    1395  &   652     \\
%                                   & GCN + Term Walks          &    1549	    &     660     &   1394       &    611         \\
%                                   &  GCN + Chains + Term Walks &    1555	    &    706      &   1435       &  690       \\
% \bottomrule
% \end{tabular}
% \caption{TRAIL's performance with different vectorization methods in terms of number of proved theorems. Best results in \textbf{bold}}
% \label{tab:vect_transfer}
% \end{table*}





% \subsection{Effects of Vectorization Choice}

% The term walk and chain-based vectorization modules used by \trail  are intended to quickly extract structural features from their inputs. Though they are not tailored to any particular domain within FOL, they are clearly feature engineering. Graph neural network (GNN) approaches have been proposed as a general alternative that can lessen the need for expert knowledge by having a neural network automatically learn salient features from the underlying graph representations of logical formulas. Though GNN approaches have quickly gained traction in this domain due to the graph-centric nature of automated reasoning \cite{paliwal2019graph,WangTWD-NIPS17-deepgraph,olvsak2019property}, they have not yet clearly demonstrated that the value they provide in terms of formula representation offsets their greater computational cost when deployed in a comparison with a state-of-the-art FOL ATP.

% We view \trail as providing a framework for further testing this, as GNN-based vectorizers can be trivially substituted into \trail's operation as one of its initial vectorization modules (see Section \ref{sec:vectorization}) that feed into the computation of the neural proof state. Consequently, 
% %To determine the effectiveness of the chain-based vectorization method introduced in Section \ref{sec:vectorization},
% we performed an experiment where we varied the vectorization modules available to \trail, comparing four different ablated versions: 1) \trail using the chain-based vectorizer, 2) \trail using the term walk vectorizer \cite{JU-CICM17-enigma}, 3) \trail using a GCN-based vectorizer~\cite{kipf2016semi}, and 4) combinations of these vectorizers. For all ablations, \trail had access to the general-purpose vocabulary-independent features %(e.g., age, literal count, etc.)
% mentioned in Section \ref{sec:vectorization}. The GCN is the standard GCN described in \cite{kipf2016semi} operating over the shared subexpression forms of clauses \cite{WangTWD-NIPS17-deepgraph}.

% We report \trail's performance using both the prior \emph{best iteration performance} metric (where the train and test sets are the same) and a more standard evaluation where the train and test sets are distinct. For the latter evaluation, we use one dataset (i.e., M2k or MPTP) to train and the other to test (see next Section). Table~\ref{tab:vect_transfer} shows the performance of \trail for these two metrics on both datasets, with the distinction between the sparse vectorization modules, the GNN-based module, and all combinations of each explicitly indicated.

% \subsubsection{Performance Within Datasets}
% Examining Table \ref{tab:vect_transfer}, we see that while chain-based vectorization is weaker than term walk vectorization, the combination of the two achieves significantly better results as a whole. This suggests that they are capturing non-redundant feature sets. %which is ideal.
% Additionally, both the term-walk vectorization and the GCN are very strong on M2k, but they do not do well in every case (i.e., there seems to be something important they are not capturing). Notably, while the GCN alone provides quite reasonable performance, combining it with other vectorization modules leads to a decrease in performance; which we suspect is due to the more expensive computational cost. However, that the GCN provides a strong baseline is promising, as it required no domain-expert knowledge. %(unlike the term walk and chain features).
% Our takeaway %from this experiment 
% is that cheap vectorization methods are currently still quite useful; however, the gap between those techniques and GNN-based approaches is closing.

% \subsubsection{Generalization Across Datasets}
% \label{sec:transfer}
% Table~\ref{tab:vect_transfer} also shows the performance of \trail when trained on M2k and tested on MPTP dataset, and vice versa. In terms of transfer, the combination of chain-based and term walk vectorization produces the best results. This provides evidence that these features are reasonably domain-general (though, we again emphasize that, while M2k and MPTP are different datasets and may require different reasoning strategies, they are both generated from Mizar). Notably, there was only a 11\% loss of performance when training on MPTP and testing M2K, and a 3\% loss when training on M2k and testing MPTP2078. From this experiment we conclude that cheap structural features, though hand-engineered, are relatively domain-general, which again will make them tough for more complex approaches to beat.

%We found that \trail with only the chain-based vectorizer solved 1,473 problems on M2k and 653 on MPTP. With only the term walk vectorizer, \trail solved 1,552 problems for M2k and solved 737 problems for MPTP. For reference, \trail utilizing both vectorizers (our main approach shown in Table \ref{tab:m2k_2078}) solved 1,561 problems on M2k and 910 problems on MPTP. This is an interesting result as it shows two things: 1) while chain-based vectorization is weaker than term walk vectorization, the combination of term walks with chain-based vectorization achieves significantly better results as a whole, and 2) the term-walk vectorization of Enigma is very strong on M2k, but does not do well in every case (i.e., there seems to be some important feature it is not capturing). {\color{red}TODO: add GCN experiment, try to include combinations of GCN, herbrand, enigma ... }


% max - I was thinking ablation results in the text, then main results in tables. If we have too many tables it might get distracting
% \begin{table}[]
%  \centering
%  \footnotesize
% \begin{tabular}{lcc}
% \toprule
%                       & M2K                       & MPTP2078                    \\
% \midrule
% Conjecture Only           & --           & --                      \\ 
% % Processed Clauses Only & --           & -- \\ 
% Combined & 1,561           & 910 \\ 

% \bottomrule
% \end{tabular}
% \caption{Performance when action selection }
% \label{tab:conj_only}
% \end{table}


% {\color{red} Add experiment to compute attention over processed clauses + conjecture vs. processed clauses only vs. conjecture clauses only}



%\textcolor{red}{elaborate}
% In the table we can see that exploratory imitation consistently yields better performance overall, however, its advantage over tabula rasa is not significant. {\color{red} An analysis of problems solved by each approach shows that they mostly solved the }


% \begin{table}[]
% \centering
% \footnotesize
% \begin{tabular}{c l c c c}
% \toprule
% %\multicolumn{2}{c}{Training} & & Testing & \\
% &  & \multicolumn{3}{c}{Testing}  \\
% \cmidrule(lr){3-5}
%  & & M2k & MPTP & TPTP \\ 
% \toprule
% \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Train}} & M2k & 1,561 & 812 & 311 \\ 
% & MPTP & 1,510 & 910 & 286 \\ 
% & TPTP & 1,333 & 532 & 347 \\ 
% \bottomrule
% \end{tabular}
% \caption{Generalization across datasets when training on one dataset and testing on the other in terms of number of problems solved}
% \label{tab:transfer_exp}
% \end{table}

% \begin{table}[]
% \centering
% \footnotesize
% \begin{tabular}{c l c c}
% \toprule
% %\multicolumn{2}{c}{Training} & & Testing & \\
% &  & \multicolumn{2}{c}{Testing}  \\
% \cmidrule(lr){3-4}
%  & & M2k & MPTP2078 \\ 
% \toprule
% \multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Train}} & M2k & 1,561 & 812  \\ 
% & MPTP2078 & 1,510 & 910  \\ 
% % & TPTP & 1,333 & 532  \\ 
% \bottomrule
% \end{tabular}
% \caption{Generalization across datasets when training on one dataset and testing on the other in terms of number of problems solved}
% \label{tab:transfer_exp}
% \end{table}







% \subsection{Reward Function Choice}
% {\color{red} Add experiment to compare time-based vs. step-based rewards}



% \begin{table}[b]
%  \centering
%  \footnotesize
% \begin{tabular}{lcc}
% \toprule
%                       & M2K                       & MPTP2078                    \\
% \midrule
% Tabula Rasa           & 1,522           & 785                      \\ 
% Exploratory Imitation & 1,555           & 823 \\ 
% \bottomrule
% \end{tabular}
% \caption{3-fold cross validation performance of \trail with different training regimens in terms of number of problems solved}
% \label{tab:train_reg_exp}
% \end{table}



% \subsection{Training on Different Regimens}
% %In this experiment, we show \trail's performance when we train it  on Mizar3.2K and test its performance on the entirety of TPTP2k and vice versa. As described earlier, these two datasets have very different vocabularies.  In examining the factors that help this sort of generalization across datasets, we examine the effect of each type of training regimen.

% In this experiment, we show \trail's performance when we train with different regimens for M2k and MPTP2078. We used 3-fold cross validation to maintain distinct training and testing sets, as exploratory imitation (introduced in Section \ref{sec:train}) stochastically delegates action selection to an expert reasoner during training. This would thus give it an unfair advantage in the iteration-based setting used in our previous experiments where training and testing were intermixed. Table~\ref{tab:train_reg_exp} shows the performance of both training regimens and how much each regimen facilitates generalization. 
% In the table we can see that exploratory imitation consistently yields better performance overall, however, its advantage over tabula rasa is not significant. {\color{red} An analysis of problems solved by each approach shows that they mostly solved the }
























































% \begin{table}[]
% \centering
% \footnotesize
% \begin{tabular}{c l c c c}
% \toprule
% %\multicolumn{2}{c}{Training} & & Testing & \\
% & Training Regimen & & Testing & \\
% \cmidrule(lr){3-5}
%  & & M2k & MPTP & TPTP \\ 
% \toprule
% & Beagle & 1,543 & 742 & -- \\
% \midrule
% \multirow{2}{*}{M2k}
%                 & Tabula Rasa           &  1,561 & 812 &  311     \\
% %                & Expert Bootstrapping  & -- & -- & -- \\
%                 & Exploratory Imitation & -- & -- & -- \\
% \midrule
% %\multicolumn{1}{c}{\multirow{3}{*}{\rothead{Training on\\ TPTP}}} 
% \multirow{2}{*}{MPTP}
%                 & Tabula Rasa           &  1,510 & 910  &   286      \\
% %                & Expert Bootstrapping  &   --  &  --  & -- \\
%                 & Exploratory Imitation &   --  &  --  & -- \\
% \midrule
% \multirow{2}{*}{TPTP}
%                 & Tabula Rasa           &  1,333  &  532  &  347        \\
% %                & Expert Bootstrapping  & -- & -- & -- \\
%                 & Exploratory Imitation & -- & -- & -- \\
% %\multirow{3}{*} {\setstackgap{S}{4.05ex}\Centerstack[l]{Train}} & M2k & 1,561 & 812 & 311 \\ 
% %& 2078b & 1,510 & 910 & 286 \\ 
% %& TPTP & 1,333 & 532 & 347 \\ 
% \bottomrule
% \end{tabular}
% \caption{Performance of \trail with different training regimens in terms of number of problems solved
% }
% \label{tab:transfer_exp}
% \end{table}



% \begin{table}
%  \centering
%  \footnotesize
% \begin{tabular}{lcc}
% \toprule
%                       & M2K                       & MPTP2078                    \\
% \midrule
% ENIGMA                      & 1,552         & 737                      \\ 
% Herbrand                    & 1,473         & 653 \\ 
% GCN                         & 1,523         & 750 \\ 
% \midrule
% Herbrand + ENIGMA           & \bf 1,561         & \bf 910 \\ 
% Herbrand + GCN              & --           & -- \\ 
% ENIGMA + GCN                & 1549      & 660 \\ 
% Herbrand + ENIGMA + GCN     & 1,555           & 699 \\ 
% \bottomrule
% \end{tabular}
% \caption{TRAIL's performance using different vectorization methods, in terms of the number of proved theorems}
% \label{tab:train_reg_exp}
% \end{table}



% \begin{table}[]
% \small
% \begin{tabular}{llll}
% \toprule
%                                   &                 & \multicolumn{2}{c}{Testing} \\
% \midrule
%                                   &                 & M2K           & MPTP2078 \\
% \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Train on \\ ~~M2K\end{tabular}}      & Herbrand  & 1473          & 418      \\
%                                   & ENIGMA          & 1552          & 570      \\
%                                   & GCN             & 1523          & 712      \\
%                                   & Herbrand+ ENIGMA & \bf 1561          & \bf 812      \\
%                                   & Herbrand+ GCN    & --                  &   --    \\
%                                   & ENIGMA + GCN    & 1549                 &   --    \\
%                                   & Herbrand + ENIGMA + GCN &  1555        &  690      \\
% \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}~~Train on \\ MPTP2078\end{tabular}} & Herbrand  & 1463 & 653      \\
%                                   & ENIGMA          & 1425          & 737      \\
%                                   & GCN             & 1394          & 750      \\
%                                   & Herbrand+ENIGMA & \bf 1510          & \bf 910     \\
%                                   & Herbrand+GCN &    --       &   --    \\
%                                   & ENIGMA+GCN &           &   660    \\
%                                   & Herbrand + ENIGMA + GCN &  1435          &  699      \\
% \bottomrule
% \end{tabular}
% \caption{Generalization across datasets when training on one dataset and testing on the other in terms of number of problems solved}
% \label{tab:transfer_exp}
% \end{table}


==> sections/abstract.tex <==
\begin{abstract}%
In recent work, we introduced \trail, a novel reinforcement learning based proof guidance system that integrates with saturation based reasoners to achieve state of the art performance on automated theorem proving for learning based systems.  \trail was designed novel mechanisms to represent the state of the theorem prover, and a novel method to represent the inference selection process.  In this work, we treat \trail as a modular system with swappable components, and we perform a comprehensive evaluation of many of these components, including the reasoning engine, vectorization methods, and reward functions for learning.  In addition, we extend these components to gain a significant benefit in performance, now approaching the performance of state of the art reasoners with hand crafted strategies for theorem proving.

%Automated theorem provers have traditionally relied on manually tuned heuristics to guide how they perform proof search.
%Deep reinforcement learning has been proposed as a way to
%obviate the need for such heuristics, however, its deployment
%in %state-of-the-art saturation-based
% I took out the saturation-based specification as we present a better approach to deep rl theorem proving in general
%automated theorem proving remains a challenge.
%
%In this paper we introduce \trail, a system that
%applies deep reinforcement learning to
%saturation-based theorem proving. \trail leverages
%(a) a novel neural representation of the state of a theorem prover
%and (b) a novel characterization of the inference selection process
%in terms of an attention-based action policy.
%
%We show through systematic analysis that these mechanisms allow \trail to significantly outperform previous reinforcement-learning-based theorem provers and approach the performance of state-of-the-art traditional theorem provers on two benchmark datasets for first-order logic automated theorem proving. 
%We show through systematic analysis that these mechanisms allow \trail to significantly outperform previous reinforcement-learning-based theorem provers on two benchmark datasets for first-order logic automated theorem proving (proving around 15\% more theorems). 
\end{abstract}

%%%% OLD ABSTRACT %%%%

%\begin{abstract}%
%Automated theorem provers have traditionally relied on manually tuned heuristics to guide how they perform proof search.
%Deep reinforcement learning has been proposed as a way to obviate the need for such heuristics, however, its deployment in real-time theorem proving remains a challenge.
%In this paper we introduce \trail, a system that applies deep reinforcement learning to theorem proving to learn proof guidance strategies automatically.
%Key to \trail's design is a novel neural representation of the state of a theorem prover in terms of available inferences and observed clauses, and a novel characterization of the inference selection process in terms of an attention-based action policy.  
%We show through systematic analysis that these mechanisms allow \trail to significantly outperform previous reinforcement-learning-based theorem provers (proving around 15\% more theorems) and approach the performance of state-of-the-art traditional theorem provers on two benchmark datasets for first-order logic automated theorem proving. To the best of our knowledge, \trail is the first theorem proving system to use proof guidance strategies learned completely from scratch to achieve performance competitive  with a state-of-the-art traditional theorem prover on a standard first-order logic theorem-proving benchmark.
%%-----------------------------
%%\trail's design also allows for a deeper integration of modern learning-based techniques with the more performant saturation-style theorem provers than has yet been possible.
%%We show through systematic studies that this representation is itself responsible for the gain in performance over the state of the art.
%%In this work we introduce \trail, a reinforcement learning (RL) based system that achieves state-of-the-art performance for RL-based theorem proving. 
%%with successful completion of 1,561 problems on the M2K benchmark and 910 problems on the MPTP2078 benchmark, beating the best reinforcement learning based system plCop performance by 338 problems. 
%%Recent work has focused on interfacing reinforcement learning with tableau-based reasoners due to their relatively straightforward design. However, current state-of-the-art theorem provers are saturation-based, which makes their integration with such techniques more challenging. 
%%In this work we introduce \trail, a system that characterizes the core ideas of saturation theorem proving within a reinforcement learning framework. 
%%This allows for a deeper integration of modern learning-based techniques with the more performant saturation-style theorem provers than has yet been possible.
%%\ibrahim{I'm not sure we should motivate the work by the ease of integration only, we should  briefly mention our modeling choices and why they matter?}

%% {\color{red}Max: we should be careful here because I'm pretty sure there's better learning-based systems for these benchmarks. we're definitely the best reinforcement learning based approach.}
%\end{abstract}

==> sections/discussion.tex <==
\section{Discussion and Future Work}

\textbf{Action Space} In typical RL setups such as games, the action space is fixed, finite and does not change in each step. However, fixing the action space in theorem proving is very challenging. In our case, we opted to have actions representing the candidate clauses to be selected at each step which made that space grows and shrink as the episode progresses. Having actions as inference rules, for example, will make the action space finite and fixed. However, this will require an extra module to select which clauses to apply the rule on, and, although at a given reasoning step the number of candidate clauses is finite, the number of candidate clauses that can be produced during a proof attempt is not bounded as new clauses are constantly produced during the reasoning process. As part of our future work, we are exploring a number of techniques that can fix or limit the action space during theorem proving. 

\textbf{Reward Function} We experimented with two types of reward functions. The first one is based on the number of steps used to find a proof while the second one is based on the amount of time spent. The advantage of time-based reward is that it implicitly encapsulate all the other costs associated with picking an action such the complexity of executing  action and how much much clauses it generate. We found empirically that both types of rewards reach the same performance eventually with time-based reward converging much faster. 


\ibrahim{add future work: behavioral cloning, other RL algorithms, extension to HOL} 


==> sections/gnns.tex <==

\section{Logic Formulae Vectorization}

\trail transforms the formulas internal to the proof state into real-valued vectors.
To do this, \trail utilizes a set of $M$ vectorization modules, $\mathcal{M} = \{ m_1, \ldots, m_M \}$, that each characterize some important aspect of the clauses and actions under consideration.

% {\color{blue} 
In addition to term walks and chain-based vectorization (described next), \trail uses general purpose modules for representing clause age (the timestep at which a clause was derived), weight (the number of symbols in the clause), literal count, and set-of-support (whether or not the clause has a negated conjecture clause as an ancestor in its proof tree). 


\subsection{Sparse Vectorization}
\label{sec:vectorization}
%\subsubsection{Producing Sparse Representations}
%For compatibility with subsequent neural components, all clauses and inferences must first be transformed into real-valued, fixed-length vectors.

Sparse vectorization modules $m_k \in \mathcal{M}$ follow the same general design: given an input clause or action, $m_k$ produces a discrete, bag-of-words style vector in $\mathbb{Z}^{n_k}$, where $n_{k}$ is a pre-specified dimensionality specific to module $m_k$. As an example, consider a module intended to capture the symbols of a formula. It would map each symbol present in its input to an index ranging from $1, \ldots, n_k$. The vector representation would be created by assigning to each dimension of a sparse $n_k$-dimensional vector the number of times a symbol corresponding to that dimension appeared in the input (i.e., a bag-of-words representation). Letting $m_k(i)$ be the sparse vector for an input $i$ from module $m_k \in \mathcal{M}$, the final vector representation $v_i$ is then the concatenation of the outputs from each module. 
% , i.e. $$ v_i = \bigparallel_{k = 1}^{M} m_k(i) ~.$$
% I removed the formula above since is obvious what we mean with "the concatenation of the outputs"

%As actions are pairs of clauses and inference rules, \trail represents the clause in each action pair using the process described above and the inference rule as a one-hot encoding of size $|\mathcal{I}|$, where $\mathcal{I}$ is the set of inference rules.

This vectorization process allows \trail to trivially incorporate techniques from the large body of research on vectorization strategies for machine learning guided theorem proving \cite{bridge2014machine,KUV-IJCAI15-features}. For instance, \trail uses Enigma \cite{JU-CICM17-enigma} modules which characterize a clause in terms of fixed-length term walks (with separate modules for term walks of length $l \in \{ 1, 2, 3\}$).


%Each such module produces a one-hot vector, where each dimension of the vector represents a different value corresponding to that feature for a particular clause. For instance, given a clause with 3 literals, the literal count module would be produce a one-hot vector with its third dimension set to one and all other dimensions set to zero.
% }

%{\color{red} describe GCN formulation}

\begin{figure}
\begin{center}
\includegraphics[width=1.0\columnwidth]{figures/trail_vectorizer.pdf}
%\includegraphics[width=1.0\columnwidth]{figures/herbrand_patterns_norename.pdf}
\caption{Overview of chain and term walk vectorizers operating on the clause $q(f(g(x, y), z), g(x, y))$}
\label{fig:herbrand_templates}
\end{center}
\end{figure}

% \subsubsection{Chain-Based Vectorization}
%Figure~\ref{fig:herbrand_templates} shows an example of the vectorizer operating on a clause with a single positive literal. 
We refer to the vectorization method introduced here as \emph{chain-based vectorization}. Within \trail, it functions as one of the available vectorization modules. Its development was inspired by the way inference rules operate over clauses. Consider the resolution inference rule. Two clauses resolve if one contains a positive literal whose constituent atom is unifiable with the constituent atom of a negative literal in the other clause.
Hence, vector representations of clauses should both capture the relationship between literals and their negations and reflect structural similarities between literals that are indicative of unifiability.

Our approach captures these features by deconstructing input clauses into sets of patterns. We define a \textit{pattern} to be a linear chain that begins from a predicate symbol and includes one argument (and its argument position) at each depth until it ends at a constant or variable. The set of all patterns for a clause is then the set of all linear paths between each predicate and the constants and variables they bottom out with. Since the names of variables are arbitrary, they are replaced with a wild-card symbol, ``$\ast$''.  %indicating that the element may match with anything. 
Argument position is also indicated with the use of wild-card symbols.
%Going back to the clause in Figure~\ref{fig:herbrand_templates}, 
%As an example, for the single literal clause $q(f(g(x, y), z), g(x, y))$, we would obtain the patterns $q(f(g(\ast, \ast), \ast), \ast)$ and $q(\ast, g(\ast, \ast))$). 

We obtain a $d$-dimensional representation of a clause by hashing the linearization of each pattern $p$ using MD5 hashes~\cite{rivest1992md5} to compute a hash value $v$, and setting the element at index $v \bmod d$ to the number of occurrences of the pattern $p$ in the clause. We also explicitly encode the difference between patterns and their negations by doubling the representation size and hashing them separately, where the first $d$ elements encode the positive patterns and the second $d$ elements encode the negated patterns. Chain vectorization is intended to produce feature vectors useful for estimates of structural similarity. Figure \ref{fig:herbrand_templates} shows how chain patterns would be extracted from a clause along with term walks. 

% {\color{blue} 
The use of hashing (provided that $d$ is small enough) is partially intended to discourage the learning of symbol or pattern-specific interactions. That is, if hash collisions are sufficiently frequent, we would expect them to act as a form of regularization that inhibits the network from relying on the presence or absence of specific patterns within a clause. Ideally (though certainly not guaranteed), the network would then instead learn to rely on more holistic features like the overall structural similarity between pairs of clauses (given by the dot product of pattern feature vectors). 
%We note, however, that this is not guaranteed, and the learning of signature-specific features is still quite possible (e.g., in cases where $d$ is too large, the number of unique chains encountered is too small, etc.).
% }

%An important design decision for \trail was to rely on a combination of simple and efficient vectorizers like the pattern-based vectorizers described above, as opposed to more complex graph neural network (GNN) approaches. Though GNN-based  approaches are powerful, they introduce a noticeable additional run-time overhead (i.e., more time spent looking for a better search strategy and less time left to execute it). We contrast our approach with a graph neural network based approach in Section~\ref{sec:experiments}.
% Cite a paper that uses GCNs


%{\color{red} Even with MD5 hashing, when operating in domains with smaller vocabularies and shorter formulas it is possible (though unlikely) that vocabulary specific features could still be learned. To mitigate this, our approach systematically renames patterns prior to hashing. Specifically, a unique identifier is appended (generated from the proof attempt number) to each predicate, function, and constant (e.g. in the second proof attempt our patterns would be $q_2(f_2(g_2(\ast,\ast),\ast),\ast)$ and $q_2(\ast, g_2(\ast, \ast))$). This does not affect the underlying semantics of a problem, as each predicate, function, and constant has been renamed consistently.}

% The pattern-based vectorization procedure is intended to produce sparse feature vectors that give reasonable estimates of purely structural similarity. Through both the hashing and renaming, \trail has minimal dependence on symbol specific features. While this is certainly appealing from a transferability perspective, we note that it could also be useful when constrained to a single domain. For instance, in Mizar nearly 40\% of symbols are introduced during the translation of theories into conjunctive normal form (these are skolem constants, skolem functions, or definitional predicates) \cite{olvsak2019property}, which means that any system being applied to Mizar must be able to handle problem specific symbols that may appear only a handful of times.
% \newline
% \newline
% \noindent\textbf{Action Vectorization:}
% Since actions are pairs of clauses and inference rules, our approach represents the clause in each action pair using the process described above and represents the inference rule as a one-hot encoding of size $|\mathcal{I}|$. We write $(\mathbf{z}_{t,i}, \hat{\mathbf{c}}_{t,i})$ to denote the encoding for action $a_{t,i}$.


\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{figures/trail_arch.png}%figures/trail_policy_net_final.pdf}
\caption{Flow from sparse vectorization through the policy network}
\label{fig:network_arch}
\end{center}
\end{figure*}


\subsection{Graph Neural Networks}

The time-sensitive nature of theorem proving makes simple, fast-to-extract features like those given above quite appealing. However, such features generally carry strong assumptions as to what is and is not useful to proof search that may ultimately limit the invention of new, more effective strategies. Graph neural networks have been proposed as a means of overcoming the hand-engineering required by previous feature extraction methods, however their application to theorem proving is still relatively recent \cite{rawsonreinforced}.

In what follows, we describe the several GNN variants that are tested in this work. Though none of the methods we present are tailored to graph representations of first-order logic, it is important to determine both the strengths and deficiencies of popular GNNs as applied to this task to guide research going forward. Here we provide a fair comparison across methods by 1) using standard implementations for each GNN \cite{FeyLenssen2019}, 2) using the same underlying theorem prover across experiments, and 3) integrating each GNN into the learning architecture at the same entry point.

\subsubsection{From Logical Formulae to Graph Representation}
As in recent works ~\cite{wang2017premise, paliwal2020graph}, we also represent logical formulae as Directed Acyclic Graphs (DAGs) as illustrated in figure~\ref{fig:dag_example}. This is mainly achieved by merging, from the parse tree of a formula, nodes corresponding to the same variable or the same constant.


\begin{figure*}
\begin{center}
\includegraphics[width=.4\textwidth] {figures/alt_gcn_fig.png}%figures/trail_policy_net_final.pdf}[width=\textwidth]
\caption{DAG representation of the formula  $\forall A, B, C .\ r(A, B)\wedge\big(p(A) \vee \lnot q(B, f(A)) \vee q(C, f(A))\big)$. Only clause (sub)graphs are embedded in our system}
\label{fig:dag_example}
\end{center}
\end{figure*}


\subsubsection{Graph Convolution Neural Networks}
Graph convolutional neural networks (GCNs) \cite{kipf2017gcn}  compute the embedding of a node as an aggregation of the embeddings for its neighbor nodes.
\begin{alignat*}{2}
h_{u}^{(i)} &= \sigma \big( W^{(i)} \big( \dfrac{h_u^{(i - 1)}}{|\mathcal{N}(u)|} + \sum_{v \in \mathcal{N}(u)} \dfrac{h_{v}^{(i - 1)}}{\sqrt{|\mathcal{N}(u)||\mathcal{N}(v)|}} \big) \big)
\end{alignat*}
where $\sigma$ is a non-linearity (in this work, we use a ReLU), $\mathcal{N}(u)$ is the set of neighbors for node $u$, and $W^{(i)}$ is a learned matrix specific to the $i$-th round of updates. Following $K$ rounds of updates, the embeddings for each node are first collected into a matrix $\mathbf{H}$ and then a pooling operation is applied to generate a single vector $\mathbf{h}$ for the input graph.

\subsubsection{Relational GCNs}
% V: schlichtkrull2018modeling neither have bias as far as I see -- but they have another aggregation
Relational GCNs (R-GCNs) \cite{schlichtkrull2018modeling} extend GCNs in that they distinguish different types of relations for computing node embeddings. Specifically, they learn different weight matrices for each edge type in the graph: 
\begin{align*}
h_{u}^{(i)} &= \sigma\left(  
\sum_{r\in \mathcal{R}}
\sum_{v\in\mathcal{N}_{u,r}} %\frac{1}
{c_{u,r}}W_{r}^{(i)} h_{v}^{(i-1)} \right)
% \label{eq:rgcn}
\end{align*}
Here, $\mathcal{R}$ is the set of edge types; 
$\mathcal{N}_{u,r}$ is the set of neighbors connected to node $u$ through the edge type $r$; $c_{u,r}$ is a normalization constant;
$W_{r}^{(i)}$ are the learnable weight matrices, one per $r\in \mathcal{R}$; 
and $\sigma$ is a non-linear activation function. 

% \subsubsection{Simple Graph Convolution}
% The Simple Graph Convolution (SGC) architecture was introduced in \cite{wu2019simplifying} as a stripped-down version of the GCN that kept only the most essential components of the GCN architecture. In particular, by removing the non-linearities between layers, they could reformulate the entire GCN as a single linear transformation. For a graph \textit{G} with adjacency matrix \textbf{A}, degree matrix \textbf{D}, and the identity matrix \textbf{I} we define the normalized adjacency matrix \textbf{S} as
% \begin{alignat*}{2}
% &\textbf{S} &&= \textbf{D}^{-\dfrac{1}{2}}(\textbf{A} + \textbf{I})\textbf{D}^{-\dfrac{1}{2}} 
% \end{alignat*}
% The SGC architecture is then the repeated application of $\mathbf{S}$ to the initial node embeddings \textbf{X} and weight matrices $\mathbf{\Theta}^{(i)}$ for each of the $i \in \{1, \ldots, K\}$ layers
% \begin{alignat*}{2}
% &\textbf{H} &&= \textbf{S}^K\textbf{X}\mathbf{\Theta}^{(1)}\mathbf{\Theta}^{(2)}\ldots\mathbf{\Theta}^{(K)}
% \end{alignat*}
% A pooling operation is applied to $\mathbf{H}$ to then generate a graph-level embedding \textbf{h} for $G$.

\subsubsection{GraphSAGE}

The GraphSAGE architecture of \cite{hamilton2017inductive} is a generalization of the GCN that allows for trainable aggregation operations. In this work, the aggregation is based on mean-pooling of neighbors to a given node
\begin{alignat*}{2}
&\hat{h}^{(i)}_u &&= \sigma\big(\mathbf{W}^{(i)}_A \cdot \dfrac{1}{|1 + \mathcal{N}(u)|}\sum_{v \in \mathcal{N}(u) \cup \{u\}}h^{(i-1)}_v \big) \\
&h^{(i)}_u &&= \sigma\big(\mathbf{W}^{(i)} \cdot (h^{(i - 1)}_u \ || \ \hat{h}^{(i)}_u)\big)
\end{alignat*}
where $||$ denotes vector concatenation, $\mathbf{W}^{(i)}_A$  and $\mathbf{W}^{(i)}$ denote weight matrices specific to layer $i$, and $\sigma$ is a ReLU non-linearity. Like the GCN, the node update step is performed for each node for $K$ rounds of updates, with the final set of node embeddings being collected into the matrix $\mathbf{H}$ and then pooled to produce $\mathbf{h}$.

% \subsubsection{Graph Attention Networks}

% Graph Attention Networks (GAT) replace the standard update layers with an attention mechanism that can better capture the importance of a node's neighbors in determining that node's hidden state. The attention value for a node $u$ with neighbor $v$ is computed as
% \begin{alignat*}{2}
% &e_{uv} &&= F^{(i)}_A(\mathbf{W}^{(i)}_A h^{(i-1)}_u \ || \ \mathbf{W}^{(i)}_Ah^{(i-1)}_v) \\
% &\alpha^{(i)}_{uv} &&= \dfrac{\exp{(e_{uv})}}{\sum_{k \in \mathcal{N}(u)}\exp{(e_{uk})}}
% \end{alignat*}
% with $F^{(i)}_A$ is a feed-forward network, $\mathbf{W}^{(i)}_A$ is a learned weight matrix, and $\alpha_{uv}$ represents the standard softmax. With each neighbor's softmax value computed, the node update step is then
% \begin{alignat*}{2}
% h^{(i)}_u &= \sum_{j \in \mathcal{N}(u)} \alpha^{(i)}_{uv} \mathbf{W}^{(i)} h^{(i-1)}_v
% \end{alignat*}
% The above equations represent the single-headed attention case, however they can be trivially extended to multi-headed attention if needed. As before, all node embeddings for the $K$-th round of updates are collected into a single matrix $\mathbf{H}$, with a pooling operation then being applied to produce a vector $\mathbf{h}$ for the input graph.

\subsubsection{Graph Convolution Neural Networks With Topological Batching}
All the graph neural network approaches discussed so far do not attempt to leverage the unique DAG structure of graphs generated from logical formulae. Inspired from recent works~\cite{crouse2019improving, thost2021directed} that leverage the acyclicity of a graph, we process, evaluate and update node embeddings in the topological order of the graph. As shown in Figure~\ref{fig:topo_batch}, the update starts from the leaf nodes (blue nodes), then proceeds to green nodes, pink nodes, yellow nodes, and finally red nodes. Nodes at the same level in the topological sort (i.e., nodes with the same color) can be updated simultaneously. Thus, nodes at the same level in the topological sort can be part of the same batch. Information propagates from leaf nodes to the root node.

The update function is as follows:
\begin{align*}
\hat{h}_{u}^{(i)} &= \sigma\left(  
\textrm{LayerNorm}\left(c_{u}W^{(i)} h_{u}^{(i-1)} +
\sum_{r\in \mathcal{R}}
\sum_{v\in\mathcal{N}_{u,r}} %\frac{1}
{c_{u,r}}W_{r}^{(i)} h_{v}^{(i)} \right)\right) \\
h_{u}^{(i)} &= \hat{h}_{u}^{(i)} + h_{u}^{(i-1)} 
% \label{eq:rgcn}
\end{align*}

Here, $\mathcal{R}$ is the set of edge types; 
$\mathcal{N}_{u,r}$ is the set of neighbors connected to node $u$ through the edge type $r$; $c_{u}$ and $c_{u,r}$ are  normalization constants;
$W_{r}^{(i)}$ are the learnable weight matrices, one per $r\in \mathcal{R}$; $W^{(i)}$ is a learnable weight matrix; 
 $\sigma$ is a non-linear activation function (here tanh); and $\textrm{LayerNorm}$ is the layer normalization function~\cite{ba2016layer}.

Two important differences in the above update equations compared to relational GCN must be stressed out:
\begin{enumerate}
    \item In the computation of the intermediary embedding $\hat{h}_{u}^{(i)}$ of node $u$,  we use the node embeddings $h_{v}^{(i)}$ of neighbors $v$ of $u$ in the current iteration $i$ whereas standard relational GCN uses the embeddings $h_{v}^{(i-1)}$ from the previous iteration $i-1$. That computation also explicitly uses the node embedding of $u$ at the previous iteration $i-1$ (i.e., $ h_{u}^{(i-1)} $).
    \item We use a residual connection as shown in the second update equation: $h_{u}^{(i)} = \hat{h}_{u}^{(i)} + h_{u}^{(i-1)}$
\end{enumerate}

\begin{figure*}
\begin{center}
\includegraphics[width=.4\textwidth] {figures/top_ord_upd.png}%figures/trail_policy_net_final.pdf}[width=\textwidth]
\caption{Update staging in DAG aware GCN. Identically colored nodes are updated simultaneously, starting at leaves}
\label{fig:topo_batch}
\end{center}
\end{figure*}

For a graph $G$, to also take into account information propagation from the root to leaf nodes, we use a bidirectional embedding as follows:
\begin{alignat*}{2}
h_{u}^{(i)}(G) &= F_{BD}\big( [ h_{u}^{(i)}(G^{\uparrow}) \ || \ h_{u}^{(i)}(G^{\downarrow})] \big)
\end{alignat*}
where $F_{BD}$ is a feed-forward network with residual connections; $||$ is the concatenation operator; $G^{\downarrow}$ is the graph G with the direction of its edges reversed; $G^{\uparrow}$ is the graph G with the direction of its edges unchanged; and $ h_{u}^{(i)}(G^{\uparrow})$ and $h_{u}^{(i)}(G^{\downarrow})$ are updated embeddings of node $u$ at iteration $i$ (following the design presented above), which accumulate node embeddings towards the root and children, respectively. 

After $K$ update iterations, the final embedding of the rooted directed acyclic graph G is given as the following function of the final embedding of its root node $root$ only: 
$$\rho(\textrm{LayerNorm}(\overline{W}h_{root}^{(K)}(G)))$$

where $\overline{W}$ is a learnable weight matrix and $\rho$ is an activation function (here ReLU).

\subsubsection{Pre-training GNN Vectorizers with Premise Selection}
%While the ability for GNN-based vectorizers to capture more complex 
At first glance, GNN-based vectorizers seem better suited for logical reasoning tasks than the simpler, pattern-based vectorizers presented earlier due to their ability to better model the explicit graph structure of logical formulas. However, the added computational overhead that GNN methods incur can mean that, even if such methods lead to more intelligent proof search, proof search is still executed too slowly to solve problems. This is particularly troublesome when training a vectorizer from scratch, as an untrained network would thus be both slower to exectute and provide less effective predictions for proof guidance.

To mitigate these concerns, we explored the common practice of network pre-training (e.g., \cite{he2016deep,turc2019well}). In particular, we investigated the effect of pre-training our GNN-based vectorizers on the related task of premise selection, i.e., the task of selecting which of a set of axioms would be used in a proof of a given conjecture. Ideally, pre-training would lead to faster convergence and greater improvements to clause selection in the earlier iterations of training. For this pre-training task, we made use of the Mizar dataset~\cite{} excluding all the problems in our evaluation benchmarks (see Section~\ref{} for details). 

% older version
%One of the main challenges that faces graph vectorizers is its computational expensiveness. This happens at two levels, during reasoning where a clause need to be vectorized and at policy network training where the vectorizer parameters need to be learned. 
%To address this issue, we investigate the idea of using a vectorizer pre-trained on a relevant task. 
%In particular, we trained a %state-of-the-art
%premise selection model~\cite{crouse2019improving} on Mizar dataset~\cite{} excluding all the problems in our evaluation benchmarks (see Section~\ref{} for details). \cite{crouse2019improving} comprises a vectorizer of premise and conjecture graph formulas and a classification model that decides if the premise is relevant to the given conjecture. In this work, we use only the vectorizer to embed the various clauses.{ \color{red} Mention vocabulary mismatch?}

